EfficientRAG: Efficient Retriever for Multi-Hop Question Answering

Retrieval-augmented generation (RAG) methods encounter difficulties when addressing complex questions like multi-hop queries. While iterative retrieval methods improve performance by gathering additional information, current approaches often rely on multiple calls of large language models (LLMs). In this paper, we introduce EfficientRAG, an efficient retriever for multi-hop question answering. EfficientRAG iteratively generates new queries without the need for LLM calls at each iteration and filters out irrelevant information. Experimental results demonstrate that EfficientRAG surpasses existing RAG methods on three open-domain multi-hop question-answering datasets.

==> section/02related.tex <==
\section{Related Works}

Recently there has been a surge in LLM-powered applications, while currently LLMs are subjected to the following limitations: 
(1) LLMs can hardly remember long-tail knowledge, they may fail in detailed knowledge-intensive tasks~\cite{DBLP:conf/icml/KandpalDRWR23}.
(2) LLMs tend to have hallucinations, e.g. generating non-factual texts~\cite{DBLP:journals/corr/abs-2401-01313}.
(3) Knowledge in LLMs will be outdated and hard to update due to a high demand for computation cost and large carbon emission~\cite{DBLP:journals/corr/abs-2309-14393}.
Retrieval augmentation is a mainstream methodology to empower LLMs with an external knowledge base~\cite{DBLP:journals/corr/abs-2312-10997}. 
Industrial retrieval-augmented LLMs typically retrieve knowledge in a direct paradigm, in which knowledge is retrieved based on the input task, or input rephrased by LLM. 
